Interacting Quantum Observables: Categorical Algebra and Diagrammatics

This paper has two tightly intertwined aims: (i) To introduce an intuitive and universal graphical calculus for multi-qubit systems, the ZX-calculus, which greatly simplifies derivations in the area of quantum computation and information. (ii) To axiomatise complementarity of quantum observables within a general framework for physical theories in terms of dagger symmetric monoidal categories. We also axiomatize phase shifts within this framework. Using the well-studied canonical correspondence between graphical calculi and symmetric monoidal categories, our results provide a purely graphical formalisation of complementarity for quantum observables. Each individual observable, represented by a commutative special dagger Frobenius algebra, gives rise to an abelian group of phase shifts, which we call the phase group. We also identify a strong form of complementarity, satisfied by the Z and X spin observables, which yields a scaled variant of a bialgebra.

==> front-matter.tex <==
%
% IOP compatible version
%

\title[Interacting Quantum Observables]{Interacting Quantum Observables: \\Categorical Algebra and Diagrammatics}


\author{Bob Coecke$^1$ and Ross Duncan$^2$}
\address{
  $^1$Oxford University Computing Laboratory\\
  Wolfson Building, Parks Road, Oxford OX1 3QD, UK
}
\address{
  $^2$Laboratoire d'Informatique Quantique,  
Universit\'{e} Libre de Bruxelles\\ 
  Boulevard du Triomphe, B-1050, Bruxelles, Belgium
}
\ead{
 $^1$\mailto{coecke@comlab.ox.ac.uk}  \ 
 $^2$\mailto{rduncan@ulb.ac.be}
}

\begin{abstract}
  This paper has two tightly intertwined aims: (i) To introduce an 
  intuitive and universal graphical calculus for multi-qubit
  systems, the \zxcalculus, which greatly simplifies derivations in the
  area of quantum computation and information.  (ii) To axiomatise
  complementarity of quantum observables within a general framework
  for physical theories in terms of dagger symmetric monoidal
  categories.  We also axiomatize phase shifts within this framework.

%%%% this seems too jargonic for the  abstract
%----
%   There is a well-studied canonical correspondence between graphical
%   calculi and symmetric monoidal categories.  Within this
%   correspondence, the atomic primitives of the graphical ZX-calculus
%   exactly correspond to a pair of complementary observables within the
%   axiomatic framework. The graphical counterpart to the phase shifts
%   renders the diagrammatic language universal.

  Using the well-studied canonical correspondence between graphical
  calculi and symmetric monoidal categories, our results provide a
  purely graphical formalisation of complementarity for quantum
  observables.  Each individual observable, represented by a
  commutative special dagger Frobenius algebra, gives rise to an abelian
  group of phase shifts, which we call the phase group.  
  
  We also identify a strong form of complementarity, satisfied by the $Z$ and
  $X$ spin observables, which yields a scaled variant of a bialgebra.

%%\bB Within an intuitive diagrammatic calculus and corresponding high-level 
%%category-theoretic algebraic description we axiomatise \em
%%complementary observables \em for quantum systems described in finite
%%dimensional Hilbert spaces, and study their interaction.  We also
%%axiomatise the \em phase shifts \em relative to an observable.  The
%%resulting graphical language is expressive enough to denote any
%%quantum physical state of an arbitrary number of qubits, and any
%%processes thereof.  The rules for manipulating these result in very
%%concise and straightforward computations with elementary quantum
%%gates, translations between distinct quantum computational models, and
%%simulations of quantum algorithms such as the quantum Fourier
%%transform.  They enable the description of the interaction between
%%classical and quantum data in quantum informatic protocols.\e
%We provide an axiomatic analysis as well as a graphical calculus for a pair of complementary quantum observables described in finite dimensional Hilbert spaces. We show that such a pair of complementary observables, together with a corresponding  account on phase shifts  relative to an observable, results in a universal language for quantum computation with qubits.  This graphical language enables very concise and straightforward computations with elementary quantum
%gates, translations between distinct quantum computational models,
%simulations of quantum algorithms %such as the quantum Fourier transform.  
%%They enable the description of 
%and the interaction between classical and quantum data in quantum informatic protocols.
%\TODO{\bB I made some substantial changes here, most notably the second paragraph is stuff which wasn't here before.\e}
%
%%\bB More specifically, we rely on the previously established fact that in
%%the symmetric monoidal category of Hilbert spaces and linear maps
%%non-degenerate observables correspond to special commutative
%%$\dag$-Frobenius algebras.  This leads to a generalisation of the
%%notion of observable that extends to arbitrary $\dag$-symmetric
%%monoidal categories ($\dag$-SMC).  We show that any observable in a
%%$\dag$-SMC comes with an abelian group of phases.  We define
%%complementarity of observables in arbitrary $\dag$-SMCs and prove an
%%elegant diagrammatic characterisation thereof. We show that an
%%important class of complementary observables give rise to a
%%Hopf-algebraic structure, and provide equivalent characterisations
%%thereof. \e
%We proof an elegant diagrammatic characterization of complementarity.  But many paris of complementary observables, most notably the Z and X spin observables, turn out to obey a much stronger condition, namely a scaled version of the axioms of a bialgebra. This strong form of complementarity, to which we refer as closed complementarity, plays a key role in the corresponding graphical calculus.  We carefully analyze the additional conditions which two complementary observables need to obey in order to be subject to the ZX graphical calculus.
%
%Our analysis does not just apply to quantum theory, but to a general class of theories described in $\dag$-symmetric monoidal categories ($\dag$-SMCs), with special commutative $\dag$-Frobenius algebras playing the role of observables.  For example, we show that any observable in a $\dag$-SMC comes with an abelian group of phases.  The study of these generalized theories has established its relevance in quantum foundations, and may contribute to crafting a theory of quantum gravity.
\end{abstract}



%\tableofcontents

\maketitle

